Adversarial Risk and the Dangers of Evaluating Against Weak Attacks

This paper investigates recently proposed approaches for defending against adversarial examples and evaluating adversarial robustness. We motivate 'adversarial risk' as an objective for achieving models robust to worst-case inputs. We then frame commonly used attacks and evaluation metrics as defining a tractable surrogate objective to the true adversarial risk. This suggests that models may optimize this surrogate rather than the true adversarial risk. We formalize this notion as 'obscurity to an adversary,' and develop tools and heuristics for identifying obscured models and designing transparent models. We demonstrate that this is a significant problem in practice by repurposing gradient-free optimization techniques into adversarial attacks, which we use to decrease the accuracy of several recently proposed defenses to near zero. Our hope is that our formulations and results will help researchers to develop more powerful defenses.

==> pixeldefend_plot.tex <==
\begin{figure}[t]
\begin{center}
%
%
%
%
%
%
%
%
%
%
%
%

\begin{tikzpicture}
\begin{axis}[epsilon_sweep, ymax=1.0, width=0.5\textwidth,height=0.33\textwidth, legend style={at={(1.0,0.35)},anchor=east} ]

\addplot+[mark=*] plot coordinates
{ (2, 0.45) (4, 0.30) (8, 0.10) (16, 0.00) };
\addlegendentry{SPSA}
\addplot+[mark=square] plot coordinates
{ (1, 0.88) (2, 0.85) (4, 0.82) (8, 0.75) (16, 0.66) };
\addlegendentry{FGSM-Transfer}
\addplot+[mark=triangle] plot coordinates
{ (1, 0.85) (2, 0.84) (4, 0.82) (8, 0.75) (16, 0.64) };
\addlegendentry{PGD-Transfer}

\end{axis}
\end{tikzpicture}

\end{center}
\caption{Accuracy of PixelDefend against various attacks. While we verify that PixelDefend is robust against transfer-based attacks from the original model, the new model still has many adversarial examples, and has 10\% adversarial accuracy against a white-box adversary.}
\end{figure}


==> plot_attack_cdf.tex <==
\definecolor{color1}{rgb}{0.00, 0.00, 1.00}
\definecolor{color2}{rgb}{0.33, 0.00, 0.66}
\definecolor{color3}{rgb}{0.66, 0.00, 0.33}
\definecolor{color4}{rgb}{1.00, 0.00, 0.00}

\begin{figure}[ht!]
\begin{center}

\begin{tikzpicture}
%
\begin{axis}[width=0.47\textwidth,height=0.3\textwidth,  %
        ymin=0,ymax=1,
        xmode=log,
        ylabel=\% of successful attacks,
        xlabel=Time (model evaluations),
        legend style={font=\small, legend cell align=left, at={(0.00, 1.0)}, anchor=north west}
]

\addplot[mark=+, color1] table[x index={0}, y index={1}, y expr={\thisrowno{1} / 100}, col sep=comma] {attack_cdf.csv};
\addlegendentry{SPSA, batch 128}
\addplot[mark=+, color2] table[x index={0}, y index={2}, y expr={\thisrowno{2} / 100}, col sep=comma] {attack_cdf.csv};
\addlegendentry{SPSA, batch 512}
\addplot[mark=+, color3] table[x index={0}, y index={3}, y expr={\thisrowno{3} / 100}, col sep=comma] {attack_cdf.csv};
\addlegendentry{SPSA, batch 2048}
\addplot[mark=+, color4] table[x index={0}, y index={4}, y expr={\thisrowno{4} / 100}, col sep=comma] {attack_cdf.csv};
\addlegendentry{SPSA, batch 8192}

\end{axis}
\end{tikzpicture}


\caption{\textbf{Model evaluations before finding misclassified adversarial example}: Although attacks with larger batch sizes require longer before beginning to identify adversarial examples, over time, they more reliably identify adversarial examples. For fair comparison, attacks with smaller batch sizes uses more iterations so that the number of model evaluations is constant across attacks. We use a log scale axis since most attacks succeed significantly sooner than the maximum number of iterations.}

\label{fig:attack_cdf}
\end{center}
\vspace{-4mm}
\end{figure}

==> plot_margin_diff.tex <==
\usepgfplotslibrary{statistics}

\begin{figure}[ht]
\begin{center}

\begin{tikzpicture}
  \begin{axis}[
    scatter, axis x line=center, axis y line=center,
    %
    width=0.47\textwidth, height=0.4\textwidth,
    xlabel={$J_{\theta}^\mathrm{adv}(x)$ using PGD},
    ylabel={$J_{\theta}^\mathrm{adv}(x)$ using SPSA},
    x label style={at={(axis description cs:0.5,-0.1)},anchor=north},
    y label style={at={(axis description cs:-0.1,.5)},rotate=90,anchor=south},
    domain=-15:10,
   ]

    \addplot[only marks, mark size=1pt, opacity=0.7] table [x index=0, y index=1, scatter src=-\thisrowno{2}, col sep=comma] {comparison_scatter.csv};
    \addplot[black, domain=-14.5:10, mark=none, scatter src=explicit] coordinates {(-15, -15)[0] (10, 10)[0]};
  \end{axis}
\end{tikzpicture}

\caption{\textbf{Analysis of gradient-free masking in adversarially trained networks}: We compare the final values of the margin-based objective across different images, after using projected gradient descent or SPSA. Each point represents a single image, and is misclassified when $J_\theta^\mathrm{adv}(x) < 0$. Points close to the line $y=x$ indicate that SPSA and PGD identified similarly adversarial perturbations. Points below the line, shown in red, indicate those for which SPSA identified stronger adversarial perturbation than PGD. Overall, SPSA and PGD identify comparably adversarial perturbations, and there are few points where SPSA identifies significantly stronger adversarial perturbations than~PGD.}\label{fig:adv_train_scatter}
\end{center}
\vspace{-4mm}
\end{figure}

==> plot_pixeldefend_detection.tex <==
\usepgfplotslibrary{statistics}

\begin{figure}[ht]
\begin{center}
%

\begin{tikzpicture}
\begin{axis}[
    ytick=\empty,
    ylabel={Frequency},
    legend style={legend cell align=left, legend columns=2, font=\small, draw=none}, 
    width=0.5\textwidth, height=0.3\textwidth,
    xlabel={Bits per dimension (CIFAR-10)}]
\addplot[hist, brown, fill, opacity=0.3, draw=none, area legend] table [ y index={0}, col sep=comma] {pixeldefend_detection.csv};
\addlegendentry{Natural}
\addplot[hist, blue, fill, opacity=0.3, draw=none, area legend] table [ y index={2}, col sep=comma] {pixeldefend_detection.csv};
\addlegendentry{Non-detectable adversarial}
\addplot[hist, red, fill, opacity=0.3, draw=none, area legend] table [ y index={1}, col sep=comma] {pixeldefend_detection.csv};
\addlegendentry{Adversarial}


%
\end{axis}
\end{tikzpicture}

\vspace{-2mm}
\caption{\textbf{Detecting adversarial examples with a generative model}: While typical adversarial examples lie in low probability regions of the input space, an adversary with access to the density model can construct non-detectable adversarial examples, which are both misclassified and assigned higher likelihood than than their natural counterparts.}
%
\label{fig:pixeldefend_detection}
\end{center}
\vspace{-8mm}
\end{figure}


==> plots_combined.tex <==
%

\def\mywidth{.45\textwidth}
%
\def\myheight{0.6\textwidth}
%

%
\begin{figure*}[b!]
\centering
\begin{subfigure}{0.8\textwidth}
    \centering
    \begin{tikzpicture} 
    \begin{axis}[%
    hide axis,
    xmin=10,
    xmax=100,
    ymin=0,
    ymax=0.4,
    legend style={legend cell align=left, legend columns=3,}
    ]
    \addlegendimage{blue,mark=*}
    \addlegendentry{SPSA};
    \addlegendimage{red,mark=square}
    \addlegendentry{FGSM-Transfer};
    \addlegendimage{brown,mark=triangle}
    \addlegendentry{PGD-Transfer};
    \end{axis}
    \end{tikzpicture}
\end{subfigure}
\begin{subfigure}{\mywidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[epsilon_sweep, ymax=1.0, width=\textwidth, height=\myheight]
    
    \addplot+[mark=*] plot coordinates
    { (1, 0.07) (2, 0.00) (4, 0.00) (8, 0.00) (16, 0.00) };
    \addlegendentry{SPSA}
    \addplot+[mark=square] plot coordinates
    { (1, 0.50) (2, 0.32) (4, 0.20) (8, 0.12) (16, 0.08) };
    \addlegendentry{FGSM-Transfer}
    \addplot+[mark=triangle,brown] plot coordinates
    { (1, 0.38) (2, 0.15) (4, 0.02) (8, 0.01) (16, 0.00) };
    \addlegendentry{PGD-Transfer}
    
    \legend{}
    
    \end{axis}
    \end{tikzpicture}
    \caption{JPEG compression (ImageNet)}
    \label{fig:jpeg_curve}

\end{subfigure}%
\begin{subfigure}{\mywidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[epsilon_sweep, ymax=1.0, ylabel={}, width=\textwidth, height=\myheight, legend style={at={(1.0,0.35)},anchor=east} ]
    
    \addplot+[mark=*] plot coordinates
    { (2, 0.45) (4, 0.30) (8, 0.10) (16, 0.00) };
    \addlegendentry{SPSA}
    \addplot+[mark=square] plot coordinates
    { (1, 0.88) (2, 0.85) (4, 0.82) (8, 0.75) (16, 0.66) };
    \addlegendentry{FGSM-Transfer}
    \addplot+[mark=triangle,brown] plot coordinates
    { (1, 0.85) (2, 0.84) (4, 0.82) (8, 0.75) (16, 0.64) };
    \addlegendentry{PGD-Transfer}
    
    \legend{}
    
    \end{axis}
    \end{tikzpicture}
    %
    \caption{PixelDefend (CIFAR-10)}
    \label{fig:pixeldefend_curve}
\end{subfigure}%
\vskip\baselineskip
\begin{subfigure}{\mywidth}
    \centering
    \begin{tikzpicture}
    \begin{axis}[epsilon_sweep, ymax=1.0, ylabel={}, width=\textwidth, height=\myheight, legend style={at={(1.0,0.4)},anchor=east}
    ]
    
    \addplot+[mark=*] plot coordinates
    { (1, 0.07) (2, 0.00) (4, 0.00) (8, 0.00) (16, 0.00) };
    \addlegendentry{SPSA}
    \addplot+[mark=square] plot coordinates
    { (1, 0.75) (2, 0.75) (4, 0.76) (8, 0.79) (16, 0.74) };
    \addlegendentry{FGSM-Transfer}
    
    \legend{}
    \end{axis}
    \end{tikzpicture}

    \caption{High-level Guided Denoising (ImageNet)}
    \label{fig:hgd_curve}
\end{subfigure}
\begin{subfigure}{\mywidth}
    \centering
    \begin{tikzpicture}
    %
    %
    \begin{axis}[epsilon_sweep, ymax=1.0, ylabel={}, width=\textwidth, height=\myheight, legend style={at={(1.0,0.4)},anchor=east}]

    \addplot+[mark=*] plot coordinates
    { (1, 0.19) (2, 0.01) (4, 0.00) (8, 0.00) (16, 0.00) };
    \addlegendentry{Stochastic PGD}
    \addplot+[mark=square] plot coordinates
    { (1, 0.58) (2, 0.46) (4, 0.32) (8, 0.24) (16, 0.14) };
    \addlegendentry{Ensemble Pattern FGSM}
    \addplot+[mark=triangle] plot coordinates
    { (1, 0.49) (2, 0.36) (4, 0.17) (8, 0.03) (16, 0.04) };
    \addlegendentry{Ensemble Pattern PGD}

    \legend{}
    \end{axis}
    \end{tikzpicture}
    \caption{Stochasticity (ImageNet)}
    \label{fig:stochasticity_curve}
\end{subfigure}

\vspace{-1.5mm}
\caption{Models can be obscured to gradient-based and transfer-based attacks by adding effectively non-differentiable operations and using purification to change the model's decision boundaries compared to the original model. However, this does not remove all adversarial examples -- using stronger attacks, we can reduce the accuracy of all defenses to near zero.}
\label{fig:combined_curves}
\vspace{-4mm}
\end{figure*}


==> summary_table.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\renewcommand\theadfont{}

\begin{table*}[t] \centering
%
%
%
%
\begin{tabular}{cp{0.38\linewidth}ccc}

\toprule
\textbf{\hphantom{0} Dataset \hphantom{0}} & \textbf{Defense strategy} & \thead{\textbf{Original} \\ \textbf{Evaluation}} & \thead{\textbf{Adversarial} \\ \textbf{Accuracy Bound}} & \thead{\textbf{Obscurity} \\ \textbf{Bound}} \\ [2pt] %
%
\midrule
%
\multirow{2}{*}{\makecell{CIFAR-10 \\ ($\epsilon=8$) }} & PixelDefend \cite{song2017pixeldefend} & 75\% & <10\% & >65\%\\ %
                          & Adversarial Training \cite{madry2017towards} & 47\% & <47\% & >0\% \\ %
\midrule
\multirow{3}{*}{\makecell{ImageNet \\ ($\epsilon=2$) }} & Non-differentiability \cite{guo2017countering} & 15\% & 0\% & 15\% \\ %
                          & Stochasticity \cite{xie2017mitigating} & 36\% & <1\% & >35\% \\ %
                          & High-level Guided Denoiser \cite{liao2017defense} & 75\% & 0\% & 75\% \\
\bottomrule
\end{tabular}

\caption{\textbf{Summary of results.} We find that while most proposed defenses confer significant robustness to the adversaries they are evaluated against in the original papers, they remain highly vulnerable to adversarial examples. Perturbation sizes $\epsilon$ are relative to images with pixel intensities in $[0, 255]$. Note that our numbers in the left column differ slightly from those in the original papers due to standardizing evaluation conditions across defenses. We explain the sources of these differences, compared to the pure replication, in the corresponding subsections.} \label{fig:results_summary}
\vspace{-4mm}
\end{table*}
